GSHOT: Few-shot Generative Modeling of Labeled Graphs

Deep graph generative modeling has gained enormous attraction in recent years due to its impressive ability to directly learn the underlying hidden graph distribution. Despite their initial success, these techniques, like much of the existing deep generative methods, require a large number of training samples to learn a good model. Unfortunately, large number of training samples may not always be available in scenarios such as drug discovery for rare diseases. At the same time, recent advances in few-shot learning have opened door to applications where available training data is limited. In this work, we introduce the hitherto unexplored paradigm of few-shot graph generative modeling. Towards this, we develop GSHOT, a meta-learning based framework for few-shot labeled graph generative modeling. GSHOT learns to transfer meta-knowledge from similar auxiliary graph datasets. Utilizing these prior experiences, GSHOT quickly adapts to an unseen graph dataset through self-paced fine-tuning. Through extensive experiments on datasets from diverse domains having limited training samples, we establish that GSHOT generates graphs of superior fidelity compared to existing baselines.

==> RelatedWork.tex <==
\begin{comment}
\section{Related Work}\vspace{-0.1in}
% We split the discussion into the two threads of graph generative modeling and few-shot learning.
\subsection{Deep Graph Generative Modelling}\vspace{-0.1in}
Several learning-based paradigms have been proposed for graph generative modeling. The first paradigm is encoder-decoder based where first graphs are encoded to a latent space and adjacency matrices are sampled to generate graphs given this latent space~\cite{graphvae,flam2020graph}. The second category is based upon deep auto-regressive models~\cite{graphrnn, goyal2020graphgen,deepgmg,gran}. These techniques generate graphs in a sequential fashion and the decision to generate the next node and edge depends upon the previous decisions. Hence, these approaches are naturally able to model the complex dependencies between the generated edges of the graph.
Among the works which are domain agnostic, DGMG~\cite{deepgmg} was one of the first approaches which learns to predict the sequence of nodes and edges of a graph. \graphRNN is an auto-regressive model that uses a BFS based node ordering strategy for generating sequences of graphs.% It utilizes a hierarchical Recurrent Neural Networks(RNNs) structure: node-based RNN and edge-based RNN to model these sequences. 
\graphGen~\cite{goyal2020graphgen} is a domain-agnostic labeled graph generation technique. It first converts graphs to unique minimum DFS codes(sequences) whose distribution is then learned through an LSTM. Owing to the unique one-to-one canonical mapping between graph and its sequence, \graphGen shows massive scalability on the domain-agnostic labeled graph generative task. For a detailed survey on graph generative modeling refer~\cite{faez2021deep}.
%  \begin{figure}[t]
%  \vspace{-0.10in}
%   \centering
%   % include first imag
%   \includegraphics[width=0.5\linewidth, height =2.5in]{samples/figures/framework.PNG}  
%   \vspace{-0.15in}
%   \caption{The pipeline of steps in \namemodel.}
%   \label{fig:framework}
% \vspace{-0.15in}
% \end{figure}
% \vspace{-0.05in}
\subsection{Few-shot learning}\vspace{-0.1in}
Few shot learning paradigm has again traction in various fields, especially where training data is scarce. The main idea is to leverage prior learning experiences and quickly adapt to a problem with a low volume of training data. There is a large body of research on few-shot learning to tackle this scenario~\cite{finn2017model, nichol2018reptile, zhou2019meta, vinyals2016matching, snell2017prototypical}.% Several techniques have been proposed to tackle this scenario.
% Examples include model-agnostic meta-learning \textsc{MAML}~\cite{finn2017model} which trains on a distribution of tasks in order to optimize its capacity to fine-tune on an unseen task. Another example is Reptile~\cite{nichol2018reptile}, which is a scalable and memory-efficient first-order gradient-based method for meta-learning.  
 We refer to the following survey~\cite{wang2020generalizing} for details. Recently, few-shot learning has also shown promising results in generative modeling tasks such as image generation in low-data regimes~\cite{lake2011one, bartunov2018few} and few-shot language tasks such as \hbox{GPT-3}~\cite{gpt}.

\vspace{-0.05in}
\subsection{Curriculum and Self-paced learning}
Curriculum learning emphasizes upon specifying an ordering of the  training instances in a computation learning setup. Inspired from the human way of learning, the key idea is to train on easy instances first and progressively incorporate difficult training samples. Several works have shown that imposing these types of orderings can improve the performance of neural models\cite{bengio2015scheduled, hacohen2019power, graves2017automated, jiang2015self}. In most of the curriculum learning techniques, a curriculum is assumed to be given by an oracle beforehand, which may or may not be easy to obtain.
% \cite{bengio2015scheduled} proposed a scheduled curriculum learning based approach for sequence prediction task by slowly increasing the difficulty of training data samples, effectively  achieving higher performance. 
The concept of self-paced learning (SPL)~\cite{jiang2015self} alleviates this  difficulty of a readily computable measure of easiness or hardness of a training sample. SPL dynamically generates the curriculum itself and adjusts the learning pace according to what the learner has already learned.
For a detailed survey on curriculum learning, we refer the reader to~\cite{soviany2021curriculum}.
\end{comment}
